Hardware Accelerator and Neural Network Co-Optimization for Ultra-Low-Power Audio Processing Devices

The increasing spread of artificial neural networks does not stop at ultralow-power edge devices. However, these very often have high computational demand and require specialized hardware accelerators to ensure the design meets power and performance constraints. The manual optimization of neural networks along with the corresponding hardware accelerators can be very challenging. This paper presents HANNAH (Hardware Accelerator and Neural Network seArcH), a framework for automated and combined hardware/software co-design of deep neural networks and hardware accelerators for resource and power-constrained edge devices. The optimization approach uses an evolution-based search algorithm, a neural network template technique, and analytical KPI models for the configurable UltraTrail hardware accelerator template to find an optimized neural network and accelerator configuration. We demonstrate that HANNAH can find suitable neural networks with minimized power consumption and high accuracy for different audio classification tasks such as single-class wake word detection, multi-class keyword detection, and voice activity detection, which are superior to the related work.

==> sections/datasets.tex <==
% !TEX root = ../hannah_iccad21.tex
\subsection{Datasets}
%HANNAH supports different datasets from three distinct domains using sensors providing \sout{1-dimensional} time-series: human speech, activity detection and electrocardiogram.
For this work HANNAH has been applied to KWS, WWD, and VAD applications. For KWS we use the Google Speech Commands Datasets V2 (GSCD) \cite{warden2018speech} 
with 10 classes for keywords ``yes," ``no," ``up," ``down," ``left," ``right," ``on," ``off," ``stop," and ``go") and 1 class for ``silence" and ``unkown", respectively.
For VAD the UW/NU Corpus 2.0 \cite{mccloy2018gender}, which contains only voice, together with the TUT Acoustic Scenes 2017 dataset \cite{mesaros2017dcase} for noise augmentation is used.
For WWD the ``Hey Snips" \cite{coucke2019efficient} dataset which contains only the eponymous word is used. % The validation and test datasets are already augmented with a noise of \SI{5}{\decibel} SNR. 

%Short discription of the following datasets and handling. Purpose of dataset, Classes, number of samples, typical division of train, validation and test dataset.
%\begin{enumerate}
%    \item GSCD \cite{warden2018speech} (v1, v2)
%    \item PAMAP2 \cite{reiss2012introducing} - Cross-Validation
%    \item "Hey Snips" \cite{coucke2019efficient} or https://research.snips.ai/datasets/keyword-spotting
%    \item MIT-BIH Atrial Fibrillation Database \cite{moody1983new} \cite{goldberger2000physiobank}
%    \item VAD - Different Variants (UW/NU Corpus 2.0 \cite{mccloy2018gender} or https://depts.washington.edu/phonlab/projects/uwnu.php, Mozilla Common Voice \cite{ardila2019common} (english, german, italian, spain, ...) )
%    \item Noise - Different Variants  ("TUT" \cite{mesaros2017dcase}, "FSDKaggle2018 \cite{fonseca2018general}", "FSDnoisy" \cite{fonseca2019learning}, FSD50K \cite{fonseca2020fsd50k})
%    \item Kitty, Cifar10 - Wäre inzwischen ja auch vorhanden. Nehmen wir den mit auf?
%\end{enumerate}

\subsection{Data Augmentation}
We augment our data with selection of a section of input, time shifts, and the addition of noise. This should lead to a more general model that can also handle noisy environments.
The selection of a section is used for all applications and is done to select a short piece of input corresponding to the length of the receptive field of the neural network. There are the three different ways to retrieve the sections: loudest part, beginning, and random. 
The mode loudest part is used to extract the loudest part of an audio recording. The mode beginning extracts the piece from the beginning of the audio recording. Both modes ensure that the input size is preserved. 
The random mode is used to randomly extract a part of the audio recording. For KWS and WWD the loudest part and for VAD a random part of the audio file is used. %The modes can also be switched in both cases.

%The random mode is a bit more complicated. From the given audio recording $y$ a section $x$ should be extracted. The length of the section $x$ is the target length.
%Three states are distinguished. If $len(y) \leq len(x)$ then the excerpt is $y$, because $y$ is too small. If $0.8len(y) \leq len(x)$ then the random piece is extracted from $y$ and has no borders.
%If $0.8len(y) > len(x)$ then the very left and right \SI{10}{\percent} of the data from $y$ are ignored and the random selection takes place between these \SI{10}{\percent} borders. This distinction is made so that, the random piece is taken in the middle area of the audio recording and not at the beginning or end of a recording because usually at the beginning or end of a recording no voice is heard yet.

The time shifts move the audio data backward or forward by a random value in a predefined interval. The data gets padded with $0$ to restore the original data size. The 
same time shifts and input section selection are used for train, test and validation. Time-shifting allows the neural network to run at a lower frequency, we use this for idle time 
optimization.  

A signal-to-noise (SNR) ratio controls the noise addition to the clean dataset. In the training phase, the SNR is randomly selected from a given interval whereas for the validation and test phase the SNR value is fixed to the desired value.


==> sections/features.tex <==
% !TEX root = ../hannah_iccad21.tex


\subsection{Quantization-Aware Training}

Many approaches to neural network quantization \cite{jacob_quantization_2018} take
a neural network trained on floating-point data and simply quantize the weights 
to integers. This approach can provide surprisingly high accuracies, but best 
results are achieved by taking the quantization effects into account during training. 

%\begin{figure}[!t]
% 	\centering
%% 	\includegraphics[width=0.46\textwidth]{figures/palom2.pdf}
%    \missingfigure[figwidth=0.9\columnwidth]{Quantization aware Training}
% 	\caption{Quantization-aware training.}
% 	\label{fig:qat}
%\end{figure}

For this, we use quantization-aware training  \cite{jacob_quantization_2018}. 
Weights, biases, and activations are quantized using a simulated quantization 
function. A floating-point value $v$ is transferred to its simulated $n$-bit 
quantized representation $v_q$ using a quantization function: HANNAH uses 
symmetric fixed-point quantization. The values are quantized according to: 

\begin{equation}
v_q = \frac{\max(\min(\mbox{round}(v\ \cdot\ 2^{n-1}), 2^{n-1}-1), -2^{n-1})}{2^{n-1}}.
\end{equation}


%\begin{enumerate}

%	\item 
%	\item Power-of-2 with Zero Quantization \cite{}:
%
%	\begin{equation}
%	v_q\ =\
%   		\begin{cases}
%		\text{sign}(v)\ \cdot 2^{-1} & \text{if} \ \log_2|v|\ \ge\ 2^{-1} \\
%		\text{sign}(v)\ \cdot\ 2^{\text{round}(\log_2(|v|))} & \text{if}\ \log_2|v|\ \ge\ 2^{n-1}\\
%   		0 & \text{otherwise} \\
%   \end{cases}
%   \end{equation}
%\end{enumerate}

At inference time, quantized values are used. Quantization effects are only simulated during the forward phase of the training. During backpropagation we adopt the straight through estimation approach \cite{bengio_ste_2013,penghang_ste_2019}, replacing quantization functions with identity functions and updating the floating-point values of weights directly. 
This allows small updates of weights to accumulate over multiple minibatches even if a single update would be too small to affect the quantized weights.

\subsubsection{Batch Norm Folding}

%\begin{figure}[!t]
% 	\centering
%    \missingfigure[figwidth=0.9\columnwidth]{Batch norm folding}
% 	\caption{Quantization-aware batch norm folding.}
% 	\label{fig:bn_folding}fig
%\end{figure}

Batch normalization is an important operation at training time, as it allows 
a faster convergence and better generalization of the trained neural networks. 
During inference, batch normalization can be reduced to a channel-wise multiplication 
and addition of constant values, which can be fused with the weights and bias of 
a preceding layer. To allow this batch norm folding, we train the neural 
network applying fake quantization on the folded weights, which allows batch 
norm folding without loss of accuracy.  

\subsubsection{Noisy Quantization}

%\begin{figure}[!t]
%	\centering
%   \missingfigure[figwidth=0.9\columnwidth]{Quantization noise}
%	\caption{Quantization noise for improved convergence of quantization aware training}
% \label{fig:noisy_qat}
%\end{figure
%}

\begin{comment}

Quantization-aware training using straight through estimation is known to work sufficiently well 
in practice for many applications, but ignoring the quantization effects during the backpropagation 
phase of training can lead to suboptimal results especially when used on very low word widths. A promising 
technique to improve convergence of low word width models in quantization-aware training is handling 
quantization as a source of noise \cite{fan2020training}.  

In this approach the quantization 
is not activated for the full training but randomly activated for each 
value with probability $p_\text{qant}$. This allows the network to partially 
learn on true floating-point values while still being resistant to quantization 
errors. In contrast to  \cite{fan2020training}, where quantization noise 
is only used to train the network weights, we use it on weights, bias, and 
activations, and integrate it with batch norm folding by applying the 
quantization noise on the folded weights.  
\end{comment}

\subsection{Neural Network Search Space}

From the use of a NAS for a specialized neural processing unit (NPU) follows the necessity of 
dynamically creating new networks of the same archetype. This is solved by configuration files
that are automatically created by the search algorithm and which are representing a valid member 
of the neural network search space. These configurations are then translated into a PyTorch model by HANNAH.
To ensure that the patterns that characterize the TC-ResNet are preserved during NAS, its configuration is 
constrained, mainly by grouping its layers into so-called major and minor blocks, where every major block 
consists of multiple minor blocks and the archetype itself consists of any number of major blocks.
\figurename{~\ref{fig:graph}} gives an overview of such a major block and shows another aspect of the 
TC-ResNet: the residual connections that split and reconnect the forwarding path.
The residual connection in \figurename{~\ref{fig:graph}} is represented by the two parallel forwarding paths
 which split before minor block 1 and 3 and reconnect after minor block 2 and 3 again.
The corresponding configuration for the network snippet in \figurename{~\ref{fig:graph}} is shown 
in \figurename{~\ref{fig:uml}}.

The attribute \textit{output channels} defines how many channels the sample should have after this major block. 
The layers of the minor block will automatically adapt to fit this number. The attribute \textit{stride} is the stride 
of the convolution filter over the weights of the sample. It only affects the first convolutional layer 
of each branch, the subsequent layers will always have stride 1. The attribute \textit{branch} defines how the forwarding path
changes if the attribute \textit{parallel} in the minor blocks is set to \texttt{true}: if \textit{branch} 
is \texttt{residual} then all parallel minor blocks form a single sequence. If \textit{branch} is \texttt{input}, 
then each parallel minor block opens its own parallel forwarding branch. If \textit{branch} is \texttt{forward} each
the attribute \textit{parallel} is ignored and the minor blocks form a simple feed-forward subnetwork. The attribute 
\textit{size} is the filter size of the 1D convolution. The further attributes \textit{padding}, \textit{batchnorm}, 
and \textit{activation} define, whether the respective operations are enabled for the corresponding minor block.

The networks use a final fully connected layer as classification head. This layer is not part of the search space as its 
input and output dimensions are determined by the number of output channels of the 
last convolutional layer and the number of classes in the dataset. Quantization parameters like word width are part of 
the neural network architecture search space. 



\begin{comment}
\subsection{Knowledge Distillation}
When training neural networks with HANNAH, different forms of knowledge distillation can be applied:
\begin{description}
	\item[Technique A]\hfill \\
	
	\item[Technique B]\hfill \\
	
	\item[Densely Guided Knowledge Distillation]\hfill \\
	The idea of Densely Guided Knowledge Distillation (DGKD) is taken from the paper in \cite{son2020densely}.
	The core idea is to have a teacher (T) and multiple teacher assistants (TAs) which sizes converge to the model size of the student and where the student loss is computed dependent on the logits of the T and TAs.
	The benefit of DGKD is that its particular computation of the student loss can prevent teacher and teacher assistants errors from adding up. %todo cite computation
	For the example of TC-ResNet this could mean that training a TC-ResNet4 with DGKD requires TC-ResNet6, -8, -14, -16 and -20 as teachers. %TODO fit example to made experiment
	%TODO dgkd figure?
	%TODO dgkd results?
\end{description}
\end{comment}




